Understanding the Representation Power of Graph Neural Networks in Learning Graph Topology

To deepen our understanding of graph neural networks, we investigate the representation power of Graph Convolutional Networks (GCN) through the looking glass of graph moments, a key property of graph topology encoding path of various lengths. We find that GCNs are rather restrictive in learning graph moments. Without careful design, GCNs can fail miserably even with multiple layers and nonlinear activation functions. We analyze theoretically the expressiveness of GCNs, concluding a modular GCN design, using different propagation rules with residual connections could significantly improve the performance of GCN. We demonstrate that such modular designs are capable of distinguishing graphs from different graph generation models for surprisingly small graphs, a notoriously difficult problem in network science. Our investigation suggests that, depth is much more influential than width, with deeper GCNs being more capable of learning higher order graph moments. Additionally, combining GCN modules with different propagation rules is critical to the representation power of GCNs.

==> misc/newcommands.tex <==
\usepackage{bm}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{color}

\newcommand*\diff{\mathop{}\!\mathrm{d}}

\newcommand{\loss} {\mathcal{L}}
\newcommand{\W} {\mathcal{W}}

\newcommand\smallO{
	\mathchoice
	{{\scriptstyle\mathcal{O}}}% \displaystyle
	{{\scriptstyle\mathcal{O}}}% \textstyle
	{{\scriptscriptstyle\mathcal{O}}}% \scriptstyle
	{\scalebox{.7}{$\scriptscriptstyle\mathcal{O}$}}%\scriptscriptstyle
}

%\newcommand{\R}{{\mathbb R}}   %% mathbb not working?
\newcommand{\E}{{\mathbb E}}   %% mathbb not working?

\newcommand{\skt}{{\mathcal{S}}}
\newcommand{\tr}{{\text{tr}}}
\newcommand{\vt}{{\text{vec}}}


\newcommand{\eat}[1]{}
%\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}


% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{fact}[theorem]{Fact}
% \newtheorem{corollary}[theorem]{Corollary}

%\newenvironment{proof}[1][Proof]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{definition}[1][Definition]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
% \newenvironment{example}[1][Example]{\begin{trivlist}
% \item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
% \newenvironment{remark}[1][Remark]{\begin{trivlist}
% \item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

%
%\newcommand{\qed}{\nobreak \ifvmode \relax \else
%      \ifdim\lastskip<1.5em \hskip-\lastskip
%      \hskip1.5em plus0em minus0.5em \fi \nobreak
%      \vrule height0.75em width0.5em depth0.25em\fi}

\newcommand{\real}{\mathbb{R}}
\newcommand{\ex}{\mathbb{E}}
\newcommand{\pq}[1]{\left( #1 \right)}
\newcommand{\Loss}{\mathcal{L}}
\newcommand{\M}[1]{{\mathbf{#1}}} % matrix
\renewcommand{\T}[1]{{\mathcal{#1}}} % tensor
\newcommand{\V}[1]{{\mathbf{#1}}} % vector
\newcommand{\SM}[1]{\mathbf{\hat{#1}}}
\newcommand{\TM}[1]{\mathbf{\bar{#1}}}
\newcommand{\krp}{\odot}
\newcommand{\PR}{\mathbb{P}}
\newcommand{\MG}[2]{\mathcal{N}(#1,#2)}
\newcommand{\OO}[1]{\mathcal{O}(#1)}
\newcommand{\OOt}[1]{\tilde{\mathcal{O}}(#1)}
\newcommand{\NI} [1]{ \N{ #1}_{1}}
\newcommand{\Nsp}[1]{ \N{ #1}_{2}}
\newcommand{\N}[1]{ {\left\| #1 \right\|}}
\newcommand{\Nf} [1]{ \N{ #1}_{\textsc{F}}}
\newcommand{\Mij}[3]{#1_{{#2},{#3}}}
\newcommand{\Mcij}[3]{{\{#1\}}_{{#2},{#3}}}
\newcommand{\SV}[2]{\sigma_{#1}(#2)}
\newcommand{\EV}[2]{\lambda_{#1}(#2)}
\newcommand{\numberthis}{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand{\abs}[1]{ {\left| #1 \right|}}

\newcommand{\ryedit}[1]{{\color{magenta} #1}}
\newcommand{\rycomment}[1]{\ryedit{[RY: #1]}}
\newcommand{\stzedit}[1]{{\color{red} #1}}
\newcommand{\stzcomment}[1]{\stzedit{[DH: #1]}}
\newcommand{\yledit}[1]{{\color{blue} #1}}
\newcommand{\ylcomment}[1]{\yledit{[YL: #1]}}


%\newcommand{\real}{\mathbb{R}}
\newcommand{\kp}{\otimes}
\newcommand{\hp}{*}
%\newcommand{\krp}{\odot}
\newcommand{\op}{\circ }
\newcommand{\cpd}[1]{{\left\llbracket {#1} \right\rrbracket}}

%\newcommand{\dhedit}[1]{{#1}}
%\newcommand{\dhcomment}[1]{}
%\newcommand{\yledit}[1]{#1}
%\newcommand{\ylcomment}[1]{}




%% ===============================================================
%% Colors
%% ===============================================================

%% ===============================================================
%% Shortcuts and symbols
%% ===============================================================

\newcommand{\doublesep}{\hspace{2pt}||\hspace{2pt}}
\newcommand{\commentthis}[1]{\begin{comment}#1\end{comment}}
\newcommand{\refn}[1]{(\ref{#1})}
\newcommand{\hsp}{\hspace{20pt}}
\newcommand{\vecc}[1]{\begin{array}\left(#1\right\end{array})}

\newcommand{\gde}[4]{\frac{\partial g_{{#1}{#2}}}{\partial {#3}^{#4}}}
\newcommand{\chr}[3]{\Gamma^{#1}{}_{#2 #3}}
\newcommand{\pderaaaa}[2]{\frac{\partial}{\partial {#1}^{#2}}}
\newcommand{\pdere}[1]{\frac{\partial^2}{\partial {#1}^2}}
% \newcommand{\tr}{\operatorname{tr}}
\newcommand{\propa}[2]{\frac{1}{#1^2-#2^2+i\epsilon}}
\newcommand{\brck}[1]{\left(#1\right)}
\newcommand{\brcksq}[1]{\left[#1\right]}
\newcommand{\brckcur}[1]{\left\{#1\right\}}
\newcommand{\brckc}[1]{\left[#1\right\}}
\newcommand{\brcka}[1]{\langle #1\rangle}
\newcommand{\norm}[1]{||#1||}

\newcommand{\bra}[1]{\langle #1|}
\newcommand{\ket}[1]{| #1\rangle}
\newcommand{\fr}[2]{\frac{#1}{#2}}
\newcommand{\vdelim}{\hspace{4pt}|\hspace{4pt}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\cl}[1]{\begin{center} #1\end{center}}

\newcommand{\lra}{\longrightarrow}
\newcommand{\lmt}{\longmapsto}
\newcommand{\llra}{\longleftrightarrow}
\newcommand{\Llra}{\Longleftrightarrow}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bali}{\begin{eqnarray*}}
\newcommand{\eali}{\end{eqnarray*}}
\newcommand{\eq}[1]{\begin{align}#1\end{align}}
\newcommand{\eqn}[1]{\begin{align*}#1\end{align*}}
\newcommand{\pmat}[1]{\begin{pmatrix}#1\end{pmatrix}}
\newcommand{\vecleft}[1]{\begin{pmatrix*}[l]#1\end{pmatrix*}}
\newcommand{\iitem}[1]{\begin{itemize}#1\end{itemize}}
\newcommand{\enumm}[1]{\begin{enumerate}#1\end{enumerate}}
\newcommand{\eps}{\epsilon}
\newcommand{\zbar}{\overline{z}}

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

\newcommand{\frakg}{\mathfrak{g}}
\newcommand{\Sym}{\trm{Sym}}
\newcommand{\mathR}{\mathbb{R}}
\newcommand{\mathC}{\mathbb{C}}
\newcommand{\mathQ}{\mathbb{Q}}
\newcommand{\mathZ}{\mathbb{Z}}

\newcommand{\tder}[2]{\frac{d #1}{d #2}}
\newcommand{\pder}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pdl}[1]{\partial_{#1}}
\newcommand{\pdu}[1]{\partial^{#1}}
\newcommand{\pd}{\partial}
\newcommand{\pdbar}{\ol{\partial}}
\newcommand{\fder}[2]{\frac{\delta #1}{\delta #2}}

\newcommand{\trm}[1]{\textnormal{#1}}
\newcommand{\tsc}[1]{\textsc{#1}}
\newcommand{\tb}[1]{\textbf{#1}}
\newcommand{\ti}[1]{\textit{#1}}

\newcommand{\mm}{\tb{m}}
\newcommand{\PP}{\tb{P}}
\newcommand{\ww}{\tb{w}}
% \newcommand{\argm}[1]{\textrm{argmax}_{#1}}
\newcommand{\argm}[1]{\textrm{argmax}_{#1}}
\newcommand{\argmi}[1]{\textrm{argmin}_{#1}}


%% ===============================================================
%% Custom commands (paper specific)
%% ===============================================================
\newcommand{\es}[1]{x_{#1}}
\newcommand{\ob}[2]{o^{#1}_{#2}}
\newcommand{\hist}[2]{h^{#1}_{#2}}
\newcommand{\ac}[2]{a^{#1}_{#2}}
\newcommand{\acc}[1]{\tb{a}_{#1}}
\newcommand{\st}[2]{s^{#1}_{#2}}
\newcommand{\stt}[1]{\tb{s}_{#1}}
\newcommand{\ep}[1]{f_{#1}}
\newcommand{\rw}[2]{r^{#1}_{#2}}
\newcommand{\rww}[1]{\tb{r}_{#1}}
\newcommand{\ms}[2]{m^{#1}_{#2}}
\newcommand{\mss}[1]{\tb{m}_{#1}}


\newcommand{\pol}[2]{\pi^{#1}_{#2}\xspace}
\renewcommand{\val}[1]{V^{#1}\xspace}
\newcommand{\ev}[1]{\mathbb{E}\brcksq{#1}\xspace}

\newcommand{\dcrnn}{\texttt{DCRNN}}
\newcommand{\trnn}{\texttt{TT-RNN}}
\newcommand{\tlstm}{TLSTM}


\newcommand{\hprod}{\odot}
\newcommand{\kprod}{\otimes}
\newcommand{\krprod}{\odot}
\newcommand{\oprod}{\circ }
\newcommand{\edges}{\mathcal{E}}
\newcommand{\graph}{\mathcal{G}}
\newcommand{\vertices}{\mathcal{V}}
\newcommand{\gconv}{{\color{red}\mathbf{\,\star_{\mathcal{G}}\,}}}
\newcommand{\bestval}[1]{{\textbf{#1}}}

==> sections/theory-bkup.tex <==
To learn graph topology, fully connected layers require a large number of hidden units.  The following theorem characterizes the representation power of fully connected neural network for learning graph moments in terms of number of nodes $N$, order of moments $p$ and number of hidden units $n$. 
% If we apply Barron's result \cite{barron1994approximation} for the universal approximator properties of fully connected neural networks to learning graph moments we find:
\begin{theorem}\label{th:barron}
A fully connected neural network with one hidden layer requires $n > O(C_f^2) \sim O(p^2 N^{2q})$ number of neurons in the best case with $1\leq q\leq 2$ 
%or $n> O(p^2 N^4) $ in the worst case 
to learn a graph moment of order $p$ for graphs with $N$ nodes.
Additionally, it also needs $S > O(nd) \sim O\pa{p^2 N^{2q+2}}$ number of samples to make the learning tractable. 
\end{theorem}
Clearly, if a FC network fully parameterizes every element in a  $N\times N$ adjacency matrix $A$, the dimensions of the input would have to be $d=N^2$. 
If the FC network allows weight sharing among nodes, the input dimension would be $d= N$. The Fourier transform of a polynomial function of order $p$ with $O(1)$ coefficients will have an $L_1$ norms of $C_f \sim O(p)$. 
Using Barron's result \cite{barron1994approximation} with $d = N^q$, where $1\leq q\leq 2$ and set the $C_f \sim O(p)$, we can obtain the approximation bound. 


In contrast to fully connected neural networks, graph convolutional networks are more efficient in learning graph moments. A graph convolution network layer without bias is of the form:
\begin{equation}
\label{eqn:GCN_layer}
    F(A,h) = \sigma(f(A)\cdot h \cdot W)
\end{equation}
Permutation invariance restricts the weight matrix $W$ to be either proportional to the identity matrix, or a uniform aggregation matrix, see Eqn. \eqref{eq:W-NPI}. 
When $W = cI$, the resulting graph moment $M_p(A)$ has exactly the form of the output of a $p$ layer GCN with linear activation function. 

% While an $n>p$ layer GCN has almost the right architecture to approximate an output of the form in \eqref{eq:moments-general}, it lacks the identity matrix term.
We first show, via an explicit example, that a  $n<p$ layer GCN by stacking layers of the form in  Eqn. \eqref{eqn:GCN_layer} cannot learn  $p$th order graph moments.
% To see the limitations in learning different functions of the graph using GCN, consider the following explicit example. 

\begin{lemma}
A  graph convolutional network with $n<p$ layers cannot, in general, learn a graph moment of order $p$ for a set of random graphs.    
\end{lemma}
We prove this by showing a  counterexample. 
Consider a directed graph of two nodes with adjacency $A= \begin{pmatrix}0 & a \\ b & 0\end{pmatrix}$. 
Suppose we want to use a single layer GCN to learn the second order moment $f(A)_i = \sum_j (A^2)_{ij} = \sum_k A_{ik} D_k$.  The node attributes $h_{il}$ are decoupled from the propagation rule $f(A)_i$. Their values are set to ones $h_{il}= 1$, or any  values independent of $A$.
The network tries to learn the weight matrix %$W_{am}$ 
$W_{l\mu}$ and has an output 
\begin{align}
    f(A)_{i\mu} &= \sigma\pa{A \cdot h \cdot W}_{i\mu} = \sigma\pa{\sum_{j,l} A_{ij} h_{jl} W_{l\mu}},
    % V_{i\mu} \equiv \sum_l h_{i} W_{l\mu} = \sum_l W_{l\mu}
    % f(A)_i& =  \sigma\pa{\sum_j A_{ij} \sum_a W_{am}} = \sigma\pa{D_i W_m}
\end{align}
For brevity, define $ V_{i\mu} \equiv \sum_l h_{il} W_{l\mu} $. 
Setting this  to the function $f(A) = A\cdot D$, which has components $f(A)_1 = f(A)_2 = ab$, and plugging in $A$, the two components become
\begin{align}
    f(A)_1 &= \sigma\pa{D_1 V_{1\mu}} = \sigma\pa{a V_{1\mu}} =ab 
    &f(A)_2 &= \sigma\pa{D_2 V_{2\mu}} = \sigma\pa{b V_{2\mu}} = ab 
    % \Rightarrow & \sigma \pa{a \sum_l h_{1l} W_{l\mu} } =  \sigma \pa{b \sum_l h_{2l} W_{l\mu} } 
\end{align}
which must be satisfied $\forall a,b $. 
Note that we don't have node attributes, so for any fixed $h_{il}$ we have
$\sigma\pa{a V_{1\mu}} = \sigma\pa{b V_{2\mu}}$. 
This states that $ \sigma(x)= \sigma(y)$ for $\forall (x,y) \in \mathbb{R}^2$, which only holds if $\sigma(\cdot)$ is a constant function, whereas $\sigma\pa{a V_{1\mu}} = ab $ implies $\sigma(x) = y$ for all $x,y$, which is impossible to satisfy by any function.
\qed{}
\outNim{
\begin{align}
    f(A)_1 &= \sigma\pa{D_1 V_\mu} = \sigma\pa{a V_\mu} =ab= \sigma\pa{b V_\mu}
      = \sigma\pa{D_2 V_\mu} = f(A)_2
    % = \sigma\pa{b W_m}\cr
    % \Rightarrow ab & = \sigma\pa{a W_m} = \sigma\pa{b W_m}= \sum A_{1j} D_j= \sum A_{2j} D_j 
    % W_\mu &\equiv \sum_l H_{il} W_{l\mu} = \sum_l W_\mu \nonumber actually, this was there already.. in 6. 
\end{align}
which should hold for any $a,b$ and $\mu$, which is  not possible. 
$\sigma\pa{a V_\mu} = \sigma\pa{b V_\mu}$ states that $ \sigma(x)= \sigma(y)$ for $\forall (x,y) \in \mathbb{R}^2$, which only holds if $\sigma(\cdot)$ is a constant function, whereas $\sigma\pa{a W_\mu} = ab $ implies $\sigma(x) = y$ for all $x,y$, which is impossible to satisfy by any function.
\qed{}
}%%%%% 

\begin{proposition}
A  graph convolutional network  with $n$ layers, and no bias terms, in general, can learn $f(A)_i = \sum_j \pa{A^p}_{ij}$ only if $n= p$ or $n>p$ if the bias is allowed.
\end{proposition}
If we use a two layer  GCN $ f(A)_i = \sum_j A_{ij} =  D_i $ to learn the  first order moment, we have  
\begin{align}
    f(A) &= \sigma_2\pa{A \cdot \sigma_1\pa{A \cdot h\cdot W^{(1)}} \cdot {W^{(2)}}} , \ 
    f(A)_1= a = \sigma_2\pa{a \sum_\mu \sigma_1\pa{b V_{2\mu}^{(1)}} {W^{(2)}}_{\mu \nu}}
\end{align}
% The proof of Lemma 1 held for arbitrary node attributes $h_{il}$. 
% By induction and replacing $h_{il}$ with the output of a GCN, we see that the same problem as above. %pathological example above leads to the multi-layer GCN failing to learn  
Again, since this must hold for any value of $a,b$ and $\nu$, the only way to satisfy this is when $\sigma_2(x) = cx$ and $\sigma_1(x W^{(1)})\cdot W^{(2)} = 1/c$, which means the output of the first layer must be constant. 
In other words, only if the first layer can be bypassed (e.g. if the bias is large and weights are zero) can a two-layer GCN learn the first order moment.  

This result also generalizes to multiple layers and higher order moments in a straightforward fashion. %, with no constraint on the activation functions.  
%Generalizing this to multilayer GCN may not look trivial when $\sigma(\cdot)$ is non-linear, but 
For GCN with linear activation, a similar argument shows that when the node attributes $h$ are not implicitly a function of $A$, in order to learn the function $ \sum_j \pa{A^p}_{ij}$, we need to have exactly $n=p$ GCN layers, without bias. With bias, a feed-forward GCN with $n>p$ layers can learn single term order $p$ moments such as 
$ \sum_j \pa{A^p}_{ij}$. 
However, since it needs to set the some weights of $n-p$ layers to zero, it can fail in learning mixed order moments such as $\sum_j (A^n+A^p)_{ij}$. 


To allow GCNs with very few parameters to learn mixed order moments, we introduce residual connections \cite{he2016deep} by concatenating the output of every layer  $h^{(m)}(A,h^{(m-1)})$ to the final output $Z[A,h] = [h_n, \dots, h_1]$ of the network. 
% \begin{align}
%     h^{(m)} &= \sigma(A\cdot h_{(m-1)} \cdot W_m+b_m) &
%     Z[A,h] &= [h_n, \dots, h_1]
% \end{align}
This way, by applying an aggregation layer or a FC layer which acts the same way on the output for every node,  we can approximate any polynomial function of graph moments. 
Specifically, the aggregation layer returns an $N\times d^o$ output of the form
\begin{align}
    Y(A,h)_{i\mu} &= \sigma\pa{\sum_{m=1}^n a^{(m)}_{\mu} \cdot h^{(m)}_i }, & h^{(m)} &= \sigma(A\cdot h^{(m-1)} \cdot W^{(m)}+b^{(m)}) ,
\end{align}
where $\cdot$ acts on the output channels of each output layers. 
The following theorem guarantees the representation power of multi-layer GCN with respect to learning graph moments.
% Additionally, a generating process may depend on moments of $\hat{A}$ or $\hat{A}_s$ defined in \eqref{eq:ops}, instead of the adjacency matrix $A$. 
% We conclude that:

% An upper bound for this error can be calculated using Barron's result \cite{barron1994approximation}, as outlined below in sec. \ref{sec:barron}. 

% \subsection{Characteristic Graph Moments}
% A graph $G$ is fully characterized by it $k$-th moments. Let's define the characteristic function of a graph as 
% % \paragraph{Dyson Series}
% % A Dyson series is a sequence defined as followed:
% $e^{\phi A} = \sum_{i=0}^\infty $

% Graph moments fully characterizes  graph generation processes. In particular, given a random graph $A$, graph moment $\E [A^p] = \E [(U\Lambda(n) U)^p] )= \E [\Lambda(n)^p])$ with fixed basis $U$. Where 

\begin{theorem}
\label{eqn:GCN_theorem}
With the number of layers $n$ greater or equal to the order $p$ of a graph moment $M_p(A)$, graph convolutional networks with residual connections can learn  a graph moment $M_p$ with $O(p)$ number of neurons, independent of the size of the graph. 
\end{theorem}
Theorem \ref{eqn:GCN_theorem} highlights the importance of residual connections. By introducing residual connections  into multiple GCN layers, we can  learn any polynomial function of graph moments.  Interestingly, Graph Isomophism Network (GIN) proposed in \cite{xu2018powerful} uses the following propagation rule:
\begin{equation}
    F(A,h) = \sigma\left(\left[ (1+\epsilon)I+ A\right]\cdot h \cdot W\right)
\end{equation}
which is a special case of our GCN design with one residual connection between two modules.  
% Next we describe a modular approach for designing GCNs that is inspired by our analysis, which significantly improve the representation power of GCNs.

% Graph Neural Networks are designed to leverage some of the properties of graph data to tackle the explosion of parameters and data requirements that happens when using a feed-forward network.
 
% Graph Convolutional Networks (GCN) \cite{kipf2016semi,defferrard2016convolutional} are designed to be explicitly node permutation invariant. 

% Similar to how a convolutional neural network exploits translation invariance (e.g. a feature can appear at any position in an image) 

% {\color{red} Check difference between GraphSAGE and GCN}


% \subsection{Expressiveness in Learning Graph Moments \label{sec:barron}}
% Learning problems over graph-structured data can be tricky.  Consider a supervised learning problem where the inputs are $N\times N$ graph adjacency matrices $A$, with components $A_{ij}$ indicating the weight of the edge going from node $i$ to node $j$.
% Assume we have $d^o$ labels $y$, meaning that we want to learn the function $\phi: R^{N^2} \to R^{d^o}$. 


% A graph convolutional neural network represents a function $G(A,h; W)$  given an adjacency matrix $A$ and node features $h$ as input and parameters $W$. 



% \begin{wrapfigure}{r}{.4\textwidth}       
%     % \begin{subfigure}[b]{0.3\textwidth}
%         \centering
%         \includegraphics[width=.4\textwidth]{figures/GCN-module-residual.pdf}
%         \caption{GCN layer (a), using three different propagation rules and a node-wise FC layer. 
%         Using residual connections (b) allows a $n$-layer modular GCN to learn any polynomial function of order $n$ of its constituent operators.}
%     % \end{subfigure}
%     \vspace{-10mm}\label{fig:residual_model}
% \end{wrapfigure}



==> sections/theory_old.tex <==
To learn graph topology, fully connected layers require a large number of hidden units.  The following theorem characterizes the representation power of fully connected neural network for learning graph moments in terms of number of nodes $N$, order of moments $p$ and number of hidden units $n$. 
% If we apply Barron's result \cite{barron1994approximation} for the universal approximator properties of fully connected neural networks to learning graph moments we find:
\begin{theorem}\label{th:barron}
A fully connected neural network with one hidden layer requires $n > O(C_f^2) \sim O(p^2 N^{2q})$ number of neurons in the best case with $1\leq q\leq 2$ 
%or $n> O(p^2 N^4) $ in the worst case 
to learn a graph moment of order $p$ for graphs with $N$ nodes.
Additionally, it also needs $S > O(nd) \sim O\pa{p^2 N^{2q+2}}$ number of samples to make the learning tractable. 
\end{theorem}
Clearly, if a FC network fully parameterizes every element in a  $N\times N$ adjacency matrix $A$, the dimensions of the input would have to be $d=N^2$. 
If the FC layer allows weight sharing among nodes, the input dimension would be $d= N$. The Fourier transform of a polynomial function of order $p$ with $O(1)$ coefficients will have an $L_1$ norms of $C_f \sim O(p)$. 
Using Barron's result \cite{barron1994approximation} with $d = N^q$, where $1\leq q\leq 2$ and set the $C_f \sim O(p)$, we can obtain the approximation bound. 


In contrast to fully connected neural networks, graph convolutional networks are more efficient in learning graph moments. A graph convolution network layer without bias is of the form:
\begin{equation}
\label{eqn:GCN_layer}
    F(A,h) = \sigma(f(A)\cdot h\cdot W)
\end{equation}
Permutation invariance restricts the weight matrix $W$ to be either proportional to the identity matrix, or a uniform aggregation matrix, see Eqn. \eqref{eq:W-NPI}. 
When $W = cI$, the resulting graph moment $M_p(A)$ has exactly the form of the output of a $p$ layer GCN with linear activation function. 

% While an $n>p$ layer GCN has almost the right architecture to approximate an output of the form in \eqref{eq:moments-general}, it lacks the identity matrix term.
We first show, via an explicit example, that a  $n<p$ layer GCN by stacking layers Eqn. \eqref{eqn:GCN_layer} cannot learn  $p$th order graph moments.
% To see the limitations in learning different functions of the graph using GCN, consider the following explicit example. 
\begin{lemma}
A  graph convolutional network with $n<p$ layers cannot, in general, learn a graph moment of order $p$ for a set of random graphs.    
\end{lemma}
We prove this by showing a  counterexample. 
Consider a directed graph of two nodes with adjacency $A= \begin{pmatrix}0 & a \\ b & 0\end{pmatrix}$. 
Suppose we want to use a single layer GCN to learn the function $f(A)_i = \sum_j (A^2)_{ij} = \sum_k A_{ik} D_k$, setting node attributes to one $h_{ia}= 1$
The network tries to learn the weight matrix $W_{am}$ and has an output 
\begin{align}
    f(A)_i &= \sigma\pa{A \cdot h \cdot W}_i = \sigma\pa{\sum_{j,a} A_{ij} h_{ja} W_{am}}, \
    W_m \equiv \sum_a h_{ia} W_{am} = \sum_a W_{am}
    % f(A)_i& =  \sigma\pa{\sum_j A_{ij} \sum_a W_{am}} = \sigma\pa{D_i W_m}
\end{align}
Setting this  to the desired function $f(A) = A\cdot D$ and plugging in $A$, we have 
\begin{align}
    f(A)_1&  = \sigma\pa{D_1 W_m} = \sigma\pa{a W_m} =ab= \sigma\pa{b W_m}
      = \sigma\pa{D_2 W_m} = f(A)_2
    % = \sigma\pa{b W_m}\cr
    % \Rightarrow ab & = \sigma\pa{a W_m} = \sigma\pa{b W_m}= \sum A_{1j} D_j= \sum A_{2j} D_j 
\end{align}
which should hold for any $a,b$ and $m$, which is  not possible. 
$\sigma\pa{a W_m} = \sigma\pa{b W_m}$ states that $ \sigma(x)= \sigma(y)$ for $\forall (x,y) \in \mathbb{R}^2$, which only holds if $\sigma(\cdot)$ is a constant function, whereas $\sigma\pa{a W_m} = ab $ implies $\sigma(x) = y$ for all $x,y$, which is impossible to satisfy by any function.
\qed{}
\begin{proposition}
A  graph convolutional network  with $n$ layers, and no bias terms, in general, can learn $f(A)_i = \sum_j \pa{A^n}_{ij}$ only if $n= p$ or $n>p$ if the bias is allowed.
\end{proposition}
If we use a two layer  GCN $ f(A)_i = \sum_j A_{ij} =  D_i $ to learn the  first order moment, we have  
\begin{align}
    f(A) &= \sigma_2\pa{A \cdot \sigma_1\pa{A \cdot h \cdot W^{(1)}} \cdot {W^{(2)}}} , \
    f(A)_1= a = \sigma_2\pa{a \sigma_1\pa{b W_m^{(1)}} {W^{(2)}}_{mk}}. 
\end{align}
Again, since this should hold for any value of $a,b$ and $k$, the only way to satisfy this is when $\sigma_2(x) = cx$ and $\sigma_1(x W^{(1)})\cdot W^{(2)} = 1/c$, which means the output of the first layer must be constant. 
In other words, only if the first layer can be bypassed (e.g. if the bias is large and weights are zero) can a two-layer GCN learn the first order moment.  

This result also generalizes to multiple layers and higher order moments in a straightforward fashion. %, with no constraint on the activation functions.  
%Generalizing this to multilayer GCN may not look trivial when $\sigma(\cdot)$ is non-linear, but 
For linear activation, a similar argument shows that when the node attributes $h$ are not implicitly a function of $A$, in order to learn the function $ \sum_j \pa{A^p}_{ij}$, we need to have exactly $n=p$ feed-forward GCN layers, without bias. With bias, a feed-forward GCN with $n>p$ layers can learn single term order $p$ moments such as 
$ \sum_j \pa{A^p}_{ij}$. 
However, since it needs to set the some weights of $n-p$ layers to zero, it can fail in learning mixed order moments such as $\sum_j (A^n+A^p)_{ij}$. 


To allow GCNs with very few parameters to learn mixed order moments, we introduce residual connections \cite{he2016deep} by concatenating the output of every layer  $h^{(m)}(A,h^{(m-1)})$ to the final output $Z[A,h] = [h_n, \dots, h_1]$ of the network. 
% \begin{align}
%     h^{(m)} &= \sigma(A\cdot h_{(m-1)} \cdot W_m+b_m) &
%     Z[A,h] &= [h_n, \dots, h_1]
% \end{align}
This way, by applying an aggregation layer or a FC layer which acts the same way on the output for every node,  we can approximate any polynomial function of graph moments. 
Specifically, the aggregation layer returns an $N\times d^o$ output of the form
\begin{align}
    Y(A,h)_{i\mu} &= \sigma\pa{\sum_{m=1}^n a^{(m)}_{\mu} \cdot h^{(m)}_i }, & h^{(m)} &= \sigma(A\cdot h_{(m-1)} \cdot W_m+b_m) ,
\end{align}
where $\cdot$ acts on the output channels of each output layers. 
The following theorem guarantees the representation power of multi-layer GCN with respect to learning graph moments.
% Additionally, a generating process may depend on moments of $\hat{A}$ or $\hat{A}_s$ defined in \eqref{eq:ops}, instead of the adjacency matrix $A$. 
% We conclude that:

% An upper bound for this error can be calculated using Barron's result \cite{barron1994approximation}, as outlined below in sec. \ref{sec:barron}. 

% \subsection{Characteristic Graph Moments}
% A graph $G$ is fully characterized by it $k$-th moments. Let's define the characteristic function of a graph as 
% % \paragraph{Dyson Series}
% % A Dyson series is a sequence defined as followed:
% $e^{\phi A} = \sum_{i=0}^\infty $

% Graph moments fully characterizes  graph generation processes. In particular, given a random graph $A$, graph moment $\E [A^p] = \E [(U\Lambda(n) U)^p] )= \E [\Lambda(n)^p])$ with fixed basis $U$. Where 

\begin{theorem}
\label{eqn:GCN_theorem}
With the number of layers $n$ greater or equal to the order $p$ of a graph moment $M_p(A)$, where  $A$ is the adjacency matrix, graph convolutional networks with residual connections can learn  a graph moment $M_p$ with $O(p)$ number of neurons, independent of the size of the graph. 
\end{theorem}
Theorem \ref{eqn:GCN_theorem} highlights the importance of residual connections. By introducing residual connections  into multiple GCN layers, we can  learn any polynomial function of graph moments.  Interestingly, Graph Isomophism Network (GIN) proposed in \cite{xu2018powerful} uses the following propagation rule:
\begin{equation}
    F(A,h) = \sigma\left(\left[ (1+\epsilon)I+ A\right]\cdot h \cdot W\right)
\end{equation}
which is a special case of our GCN design with one residual connection between two modules.  
% Next we describe a modular approach for designing GCNs that is inspired by our analysis, which significantly improve the representation power of GCNs.

% Graph Neural Networks are designed to leverage some of the properties of graph data to tackle the explosion of parameters and data requirements that happens when using a feed-forward network.
 
% Graph Convolutional Networks (GCN) \cite{kipf2016semi,defferrard2016convolutional} are designed to be explicitly node permutation invariant. 

% Similar to how a convolutional neural network exploits translation invariance (e.g. a feature can appear at any position in an image) 

% {\color{red} Check difference between GraphSAGE and GCN}


% \subsection{Expressiveness in Learning Graph Moments \label{sec:barron}}
% Learning problems over graph-structured data can be tricky.  Consider a supervised learning problem where the inputs are $N\times N$ graph adjacency matrices $A$, with components $A_{ij}$ indicating the weight of the edge going from node $i$ to node $j$.
% Assume we have $d^o$ labels $y$, meaning that we want to learn the function $\phi: R^{N^2} \to R^{d^o}$. 


% A graph convolutional neural network represents a function $G(A,h; W)$  given an adjacency matrix $A$ and node features $h$ as input and parameters $W$. 



% \begin{wrapfigure}{r}{.4\textwidth}       
%     % \begin{subfigure}[b]{0.3\textwidth}
%         \centering
%         \includegraphics[width=.4\textwidth]{figures/GCN-module-residual.pdf}
%         \caption{GCN layer (a), using three different propagation rules and a node-wise FC layer. 
%         Using residual connections (b) allows a $n$-layer modular GCN to learn any polynomial function of order $n$ of its constituent operators.}
%     % \end{subfigure}
%     \vspace{-10mm}\label{fig:residual_model}
% \end{wrapfigure}


